Stellar Streams Discovered in the Dark Energy Survey

We perform a search for stellar streams around the Milky Way using the first three years of multi-band optical imaging data from the Dark Energy Survey (DES). We use DES data covering $\sim 5000$ sq. deg. to a depth of $g > 23.5$ with a relative photometric calibration uncertainty of $< 1 \%$. This data set yields unprecedented sensitivity to the stellar density field in the southern celestial hemisphere, enabling the detection of faint stellar streams to a heliocentric distance of $\sim 50$ kpc. We search for stellar streams using a matched-filter in color-magnitude space derived from a synthetic isochrone of an old, metal-poor stellar population. Our detection technique recovers four previously known thin stellar streams: Phoenix, ATLAS, Tucana III, and a possible extension of Molonglo. In addition, we report the discovery of eleven new stellar streams. In general, the new streams detected by DES are fainter, more distant, and lower surface brightness than streams detected by similar techniques in previous photometric surveys. As a by-product of our stellar stream search, we find evidence for extra-tidal stellar structure associated with four globular clusters: NGC 288, NGC 1261, NGC 1851, and NGC 1904. The ever-growing sample of stellar streams will provide insight into the formation of the Galactic stellar halo, the Milky Way gravitational potential, as well as the large- and small-scale distribution of dark matter around the Milky Way.

==> table_names.tex <==
\begin{deluxetable}{l c}
\tablecolumns{9}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Stream Name Meanings \label{tab:names}}
\tablehead{
Name & Meaning
}
\startdata
Indus           & Indus River, India \\
Jhelum          & Jhelum River, India \\
Ravi            & Ravi River, India \\
Chenab          & Chenab River, India \\
Elqui           & Elqui River, Chile  \\
Aliqa Uma       & Aymara term for "peaceful water" \\
Turbio          & Turbio River, Chile \\
Willka Yaku     & Quechua term for "sacred water" \\
Turranburra     & Eora name for Lane Cove River, Australia \\
Wambelong       & Wambelong Creek, Australia; Gamilaraay word for "crazy water" \\
Palca           & Quechua word for "cross of rivers" \\
\enddata
{\footnotesize \tablecomments{To honor the long astronomical traditions in India, Chile, and Australia, we have named the stellar streams presented in this work after aquatic terms and rivers from these regions. The stellar streams in Q1 fall within the Indus constellation and are therefore named after the Indus river and other rivers in India. The streams in Q2 and Q3 are named after rivers in Chile and aquatic terms in native Chilean languages. The streams in Q4 are named for Aboriginal names for Australian rivers.}}
%\tablenotes
\end{deluxetable}

